Target-based Surrogates for Stochastic Optimization

We consider minimizing functions for which it is expensive to compute the (possibly stochastic) gradient. Such functions are prevalent in reinforcement learning, imitation learning and adversarial training. Our target optimization framework uses the (expensive) gradient computation to construct surrogate functions in a \emph{target space} (e.g. the logits output by a linear model for classification) that can be minimized efficiently. This allows for multiple parameter updates to the model, amortizing the cost of gradient computation. In the full-batch setting, we prove that our surrogate is a global upper-bound on the loss, and can be (locally) minimized using a black-box optimization algorithm. We prove that the resulting majorization-minimization algorithm ensures convergence to a stationary point of the loss. Next, we instantiate our framework in the stochastic setting and propose the $SSO$ algorithm, which can be viewed as projected stochastic gradient descent in the target space. This connection enables us to prove theoretical guarantees for $SSO$ when minimizing convex functions. Our framework allows the use of standard stochastic optimization algorithms to construct surrogates which can be minimized by any deterministic optimization method. To evaluate our framework, we consider a suite of supervised learning and imitation learning problems. Our experiments indicate the benefits of target optimization and the effectiveness of $SSO$.

==> Sections/RelatedWork.tex <==

{\color{red} 

\section{Additional Related Work}

% relationship to proximal point methods 
Target-space optimization is intimately related to proximal point methods~\cite{drusvyatskiy2017proximal, schmidt2011convergence}. Unlike the target optimization framework, such methods do not directly regularize in the space of targets but instead, like gradient decent, regularize directly in parameter space. Such methods often rely on composable problem structure, as in the linear-prox algorithm, which defines its proximal map using the linearized output of the model instead of the model output itself~\cite{drusvyatskiy2017proximal}. Additionally, such frameworks rarely provide guarantees in the stochastic setting. \citet{schmidt2011convergence} for instance, provides convergence in full batch settings where the proximal map is solved inexactly at each step, while our framework considers both the deterministic and stochastic setting under inexact solutions to the intermediate surrogate functions.

% relationships to proximal back-propigation
Other approaches relating proximal updates to composable losses, consider new classes of surrogate functions which are minimized (sometimes independently) at each stage of function approximation~\citep{frerix2018proximal}. Such ``layer-wise" loss construction in deep-neural networks has been shown to alleviate vanishing-gradient issues~\citep{JMLR:v22:20-1006}, and even achieve empirical performance on-par with second order methods~\citep{pmlr-v151-amid22a}. In addition to empirically improving the conditioning of the problem, many of these methods are constructed following either an implicit or explicit set of constraints between layers, which when formulated as a penalty method, allow for each sub-problem to be updated entirely independently of one another~\citep{pmlr-v48-taylor16, wang2019admm}. Such approaches however either provide no theoretical guarantees, or only consider the deterministic, full batch setting.

% relationship to approximate second-order methods 
As discussed in \cref{sec:introduction}, target based surrogate optimization can be interpreted as interpolating between first and second order methods, depending on the chosen target space and loss function. Such an approach remains distinct from previous works which attempt to directly approximate second order methods like inexact-newton~\cite{dembo1982inexact} and quasi-newton~\cite{pmlr-v5-schmidt09a}. Unlike these approaches, target space optimization provides a \textit{framework} in which one can design and analyze optimization algorithms applied to the composable and costly loss functions often found in policy optimization and deep-learning. 

% relationship to retro-opt and data-echoing.
From a technical perspective, our work functions similarly to existing analysis on direct minimization of the intermediate functions sampled in the general stochastic setting. In these examples, a set of data-points is sampled, and the function induced by the mini-batch is directly minimized over the course of k steps~\citep{agarwal2020stochastic}, or up to some tolerance criteria~\citep{biegler2004retrospective}. Like our own work, these settings are interested in improving optimization in the presence of expensive data sampling, and take advantage of so called data-echoing~\citep{choi2019faster} to improve empirical performance of the algorithm. Other more complex approaches consider a modified parametric smoothness surrogate which includes an additional ``proxy" loss term, whose second order information approximately matches the true (deterministic) loss function~\citep{woodworth2023two}. Like the other examples, this approach targets costly loss functions, but extends (with the added curvature requirement on the auxiliary loss) to areas like semi-supervised learning. 




% This question has also been answered in more complex instantiations of surrogate optimization, where an additional ``proxy-loss" is included whose curvature is sufficiently similar to the original problem of interest~\citep{woodworth2023two}.

% Like SSO, such methods also actively consider the trade-off between improvements made through using approximations of the curvature and the bias introduced through direct minimization of the function in the presence of noise~\citep{agarwal2020stochastic}. 

%  can also be viewed through the lens of approximating second order optimization algorithms, depending on the chosen surrogate and loss. Other approaches to approximating second order methods in settings where querying the (possibly stochastic) gradient oracle are expensive have been investigated in the past~\cite{pmlr-v5-schmidt09a}, . Additionally, analysis for inexact-Newton in the deterministic convex setting have also been considered~\cite{dembo1982inexact}. Unlike these approaches, the second-order behavior we observe in our framework is a byproduct of the chosen surrogate, making our analysis more widely applicable.

% other algorithms 

}



